ELF: An Early-Exiting Framework for Long-Tailed Classification

The natural world often follows a long-tailed data distribution where only a few classes account for most of the examples. This long-tail causes classifiers to overfit to the majority class. To mitigate this, prior solutions commonly adopt class rebalancing strategies such as data resampling and loss reshaping. However, by treating each example within a class equally, these methods fail to account for the important notion of example hardness, i.e., within each class some examples are easier to classify than others. To incorporate this notion of hardness into the learning process, we propose the EarLy-exiting Framework(ELF). During training, ELF learns to early-exit easy examples through auxiliary branches attached to a backbone network. This offers a dual benefit-(1) the neural network increasingly focuses on hard examples, since they contribute more to the overall network loss; and (2) it frees up additional model capacity to distinguish difficult examples. Experimental results on two large-scale datasets, ImageNet LT and iNaturalist'18, demonstrate that ELF can improve state-of-the-art accuracy by more than 3 percent. This comes with the additional benefit of reducing up to 20 percent of inference time FLOPS. ELF is complementary to prior work and can naturally integrate with a variety of existing methods to tackle the challenge of long-tailed distributions.

==> Sections/00-Planning.tex <==
\section{Planning}
\begin{itemize}
    \item  Ways to pitch our method
    \begin{itemize}
        \item CNN
        \item CNN + undersampling (2x)
        \item CNN + oversampling (3x)
        \item CNN + loss weighting (prior based)
        \item CNN + focal loss
    \end{itemize}
    
    
\end{itemize}


==> Sections/01-Introduction.tex <==
\section{Introduction}
Real world data exhibits a long tailed distribution over classes wherein only a few classes contain the majority of examples while numerous rare classes contain only a fewrelatively fewer examples. 
On datasets following this distribution, neural networks get biased towards the majority classes leading to poor generalization on rare classes.
% In such scenarios, neural networks trained on artificicially balanced datasets such as Imagenet generalize poorly. 
The problem of learning under class imbalance has conventionally been dealt either by resampling the data (undersampling, over-sampling) or by reshaping the loss function (loss reweighting, regularization). 
These approaches focus solely on the support of classes to address the challenge of class imbalance. While class support is an important consideration, relying solely on it leads us to miss an important detail - each datapoint within a particular class is treated similarly irrespective of its hardness. 
Intuitively, there might be easy examples in the minority class that get incorrectly upweighted (oversampled) or difficult examples in the majority class that get erroneously downweighted (undersampled). 
% all easy examples within a class (majority or minority) should contribute a relatively lower loss in comparison to to harder examples across all classes.
In this paper, we show that by incorporating the notion of hardness during training, we can outperform recent carefully constructed losses using traditional cross-entropy in the class imbalance setting.

Towards this goal, we propose \method{} (Figure \ref{fig:motivation}), a novel architecture which addresses the class imbalance problem by incorporating the notion of input-hardness during training. At each auxiliary exit, the neural network aims to correctly predict the input with a high score. If the prediction is incorrect, or the confidence is not high enough (typical for difficult inputs) the example proceeds to the next exit. Early-exiting \textit{during training} serves two purposes (1) It removes easy examples earlier in the inference pipeline thereby freeing up model capacity (in the later layers) for learning on harder examples and (2) The overall loss generated on easier examples is naturally lower than that of hard examples which accumulate a non zero loss at each early-exit. It must be noted that the concept of early-exiting is not new and has been widely studied previously. However the important difference is that previous works primarily leverage the idea to save compute during \textit{inference time}. In contrast, we use the idea of early-exiting \textit{during training}, specifically to tackle the problem of class imbalance.   

In the class imbalance setting, to the best of our knowledge, only Focal Loss [] incorporates the notion of hardness. They weigh the cross entropy loss $-log(p_y)$ with the prediction probability to get  $-(1-p_y) log(p_y)$. This modification allows the network to focus more on difficult examples (smaller $p_y$) whose loss contribution is larger. Notice that \method{}  can achieve a similar effect albeit through early exiting. In particular, the loss accumulated by the difficult examples at each exit, is much higher than the easy examples which contribute loss only at a few early exits. Empirically, we observe that \method{} outperforms the Focal Loss in terms of accuracy. 
\rd{Move results to contributions}
In addition since \method{} learns the notion of input-hardness during training, it can save compute essentially for free by early-exiting these examples during inference time.

\noindent
\textbf{Contributions.} Our key contributions are (i) we propose an early-exit architecture during training and inference which not only accounts for difference of class prevalance but also considers distinction of easy and hard examples within a class 
(ii) our proposed framework shows significant improvements on several object recognition datasets, such as CIFAR-10, CIFAR-100 and iNaturalist 
(iii) 

% Next, the literature related to this work is discussed.








\begin{figure}[h!]
    \includegraphics[width=\textwidth]{Images/crown.pdf}
    \caption{Early exiting neural network 
    %\scott{crisper and same sized images will make it look better; think we should also add some visually interesting patterns to the CNN blocks. Maybe from actual layers?}
    }
    \label{fig:motivation}
\end{figure}

==> Tables/dataset-statistics.tex <==
\begin{table*}[t]
\footnotesize
\setlength{\tabcolsep}{6pt}
% \centering
\begin{tabular}{llrrrrrrrrrrrrrrrrrrrr}
\toprule

& & \multicolumn{4}{c}{\textbf{CIFAR-10 LT}} & \multicolumn{4}{c}{\textbf{CIFAR-100 LT}} &
\multicolumn{4}{c}{\textbf{ImageNet LT}} &
% \multicolumn{4}{c}{\textbf{iNat'17}} & 
\multicolumn{4}{c}{\textbf{iNaturalist'18}} \\ 

\cmidrule(l){3-6}\cmidrule(l){7-10}\cmidrule(l){11-14}\cmidrule(l){15-18}\cmidrule(l){19-22}

\multicolumn{2}{c}{\textbf{Stats}} & 10 & 20 & 50 & 100 & 10 & 20 & 50 & 100 & 10 & 20 & 50 & 100 & 10 & 20 & 50 & 100 \\
%& 10 & 20 & 50 & 100 \\ 

\midrule

\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{Train}}} 
& Min & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  & 0 & 0 & 0 & 0  & 0 & 0 & 0 & 0  \\[0.5ex]

& Max & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  & 0 & 0 & 0 & 0  & 0 & 0 & 0 & 0 \\[3ex]

\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{Test}}} 
& Min & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  & 0 & 0 & 0 & 0  & 0 & 0 & 0 & 0 \\[0.5ex]

& Max & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  & 0 & 0 & 0 & 0  & 0 & 0 & 0 & 0 \\[0.5ex]

\bottomrule     

\end{tabular}
\label{table:dataset-statistics}
\caption{Dataset statistics on CIFAR-10 LT, CIFAR-100 LT, ImageNet LT and iNaturalist'18. We provide the number of images for the minority and majority classes in both the train and test splits.}
\end{table*}

==> Tables/large-datasets.tex <==
% \begin{table*}
% \setlength{\tabcolsep}{11.5pt}

% \begin{tabular}{llrrrr}
% \toprule
% \textbf{Model} & \multicolumn{1}{l}{\textbf{Method}} & \textbf{iNaturalist-18} & \textbf{ImageNet-LT} \\ 

% \midrule

% \multirow{6}{*}[-1.5ex]{\rotatebox[origin=c]{90}{\textbf{Resnet-50}}}
% & He~\cite{he2016deep} & 37.3 & 55.1\\[0.5ex]
% & Cui-D~\cite{cui2019class} & 33.9 & 51.5 \\[0.5ex]
% & Lin-D~\cite{lin2017focal} & 34.6 & 52.1 \\[0.5ex]
% & Cao-D~\cite{cao2019learning} &  32.9 & 51.2 \\[1.5ex]
% & \method-D (CE) & \textbf{33.4} & \textbf{51.2} \\[0.5ex]
% & Flops Saving (in \%) & 13.5 & 20.7 \\[0.5ex]
% & \method-D (LDAM) & ORC-3 & \textbf{49.2} \\[0.5ex]
% & Flops Saving (in \%) & - & 7.4 \\[0.5ex]

% \midrule

% \multirow{6}{*}[-1.5ex]{\rotatebox[origin=c]{90}{\textbf{Densenet-169}}}
% & Huang~\cite{huang2017densely} & 37.0 & 55.4 \\[0.5ex]
% & Cui-D~\cite{cui2019class} & 33.2 & 52.1 \\[0.5ex]
% & Lin-D~\cite{lin2017focal} & 34.5 & 52.3 \\[0.5ex]
% & Cao-D~\cite{cao2019learning} & 32.5 & 51.2 \\[1.5ex]
% & \method-D (CE) & ORC-1 & DGX \\[0.5ex]
% & Flops Saving (in \%) & - & - \\[0.5ex]
% & \method-D (LDAM) & \textbf{32.2} & \textbf{49.2} \\[0.5ex]
% & Flops Saving (in \%) & 4.4 & 1.7 \\[0.5ex]

% \bottomrule

% \end{tabular}
% \caption{Top-1 error rates (lower is better) on large scale datasets \rd{}}
% \end{table*}

% \begin{table*}[t]
% \setlength{\tabcolsep}{10pt}
% \centering
% \begin{tabular}{lllll}
% \toprule
% & \multicolumn{2}{c}{\textbf{Imagenet Long Tailed}} & \multicolumn{2}{c}{\textbf{iNaturalist18}} \\ 
% \cmidrule(l){2-3}\cmidrule(l){4-5}
% \textbf{Method} & \multicolumn{1}{l}{Resnet-50} & Densenet-169  & Resnet-50 & Densenet-169  \\ 
% \midrule
% CE & 55.4 & 55.1 &  37.3 & 37.0  \\%[0.5ex]
% % CE-DRS \cite{cao2019learning} & - &  - & 36.4 & -  \\%[0.5ex]
% LWS \cite{kang2019decoupling}  & 52.3 &   - & 34.1 & -  \\%[0.5ex]
% $\tau$-normalized \cite{kang2019decoupling} & 53.3  &  - & 34.4 & -  \\%[0.5ex]
% BBN \cite{zhou2019bbn} & - &  - & 33.7 & -  \\%[0.5ex]
% \midrule
% CE-DRW~\cite{cui2019class} & 51.5 & 52.1 &  33.9 & 33.2  \\%[0.5ex]
% Focal-DRW~\cite{lin2017focal}  & 52.1 & 52.3 &  34.6 & 34.5 \\%[0.5ex]
% LDAM-DRW~\cite{cao2019learning}  & 51.2 & 51.2 &   33.9 & 32.5 \\%[0.5ex]
% \midrule
% EEL (LDAM)-DRW   & \textbf{49.0} (-2.7) & \textbf{49.2} (-2.7) & \textbf{32.1} (-9.0) & \textbf{32.2} (-4.4)\\%[0.5ex]
% % Flops Saving (in \%) & 2.7 &  2.7 &  9.0 & 4.4   \\ 
% \bottomrule     
% \end{tabular}
% \caption{Error: Large scale experiments \rd{Change error to accuracy} \rd{Add flops in parenthesis} \rd{For BBN add flops saving will be +100 and EEL will be -10}}
% \label{tab:large_scale_results_old}
% \end{table*}

% \begin{table}[h!]
\setlength{\tabcolsep}{3pt}

% \centering
\begin{tabular}{lll}
\toprule
& \multicolumn{1}{c}{Imagenet-LT} & \multicolumn{1}{c}{iNaturalist18} \\ 
% \cmidrule(l){2-2}\cmidrule(l){3-3}
% \textbf{Method} & \multicolumn{1}{l}{Resnet-50} & Resnet-50  \\ 
\midrule
CE & 44.6 \scriptsize{(\textcolor{black}{0.00\%})} &  62.7 \scriptsize{(\textcolor{black}{0.00\%})}  \\%[0.5ex]
% CE-DRS \cite{cao2019learning} & - &  - & 36.4 & -  \\%[0.5ex]
LWS \cite{kang2019decoupling}  & 47.7  & 65.9   \\%[0.5ex]
$\tau$-norm \cite{kang2019decoupling} & 46.7  & 65.6  \\%[0.5ex]
BBN \cite{zhou2019bbn} & - & 66.3 \scriptsize{(\textcolor{red}{+100})}   \\%[0.5ex]
\midrule
CE+\scriptsize{DRW}~\cite{cui2019class} & 48.5 &  66.1  \\%[0.5ex]
Focal+\scriptsize{DRW}~\cite{lin2017focal}  & 47.9 &  65.4  \\%[0.5ex]
LDAM+\scriptsize{DRW}~\cite{cao2019learning}  & 48.8 &   66.1  \\%[0.5ex]
\midrule
EEL (\scriptsize{LDAM})+\scriptsize{DRW}   & \textbf{51.0} \scriptsize{(\textcolor{blue}{\textbf{-2.7}})}  & \textbf{67.9} \scriptsize{(\textcolor{blue}{\textbf{-9.0}})} \\%[0.5ex]
% Flops Saving (in \%) & 2.7 &  2.7 &  9.0 & 4.4   \\ 
\bottomrule     
\end{tabular}

% \caption{Top-1 accuracy for various models trained on long tailed Imagenet and iNaturalist'18 datasets. Numbers in parenthesis indicate the flops expended by each method relative to the baseline. Whenever absent, assume 0\% flops saving. \method consistently improves accuracy while expending fewer flops. }
% \label{tab:large_scale_results}
% \end{table}



% % \begin{table}[h!]
% \setlength{\tabcolsep}{1pt}

% % \centering
% \begin{tabular}{lllll}
% \toprule
% & \multicolumn{2}{c}{\textbf{Imagenet Long Tailed}} & \multicolumn{2}{c}{\textbf{iNaturalist18}} \\ 
% \cmidrule(l){2-3}\cmidrule(l){4-5}
% \textbf{Method} & \multicolumn{1}{l}{Resnet-50} & Densenet-169  & Resnet-50 & Densenet-169  \\ 
% \midrule
% CE & 44.6 \scriptsize{(\textcolor{black}{0.00\%})} & 44.9 \scriptsize{(\textcolor{black}{0.00\%})} &  62.7 \scriptsize{(\textcolor{black}{0.00\%})} & 63.0  \scriptsize{(\textcolor{black}{0.00\%})} \\%[0.5ex]
% % CE-DRS \cite{cao2019learning} & - &  - & 36.4 & -  \\%[0.5ex]
% LWS \cite{kang2019decoupling}  & 47.7 &   - & 65.9 & -  \\%[0.5ex]
% $\tau$-normalized \cite{kang2019decoupling} & 46.7  &  - & 65.6 & -  \\%[0.5ex]
% BBN \cite{zhou2019bbn} & - &  - & 66.3 \scriptsize{(\textcolor{red}{+100})} & -  \\%[0.5ex]
% \midrule
% CE+\scriptsize{DRW}~\cite{cui2019class} & 48.5 & 47.9 &  66.1 & 66.8  \\%[0.5ex]
% Focal+\scriptsize{DRW}~\cite{lin2017focal}  & 47.9 & 47.7 &  65.4 & 65.5 \\%[0.5ex]
% LDAM+\scriptsize{DRW}~\cite{cao2019learning}  & 48.8 & 48.8 &   66.1 & 67.5 \\%[0.5ex]
% \midrule
% EEL (\scriptsize{LDAM})+\scriptsize{DRW}   & \textbf{51.0} \scriptsize{(\textcolor{blue}{\textbf{-2.7}})} & \textbf{50.8} \scriptsize{(\textcolor{blue}{\textbf{-2.7}})} & \textbf{67.9} \scriptsize{(\textcolor{blue}{\textbf{-9.0}})} & \textbf{67.8} \scriptsize{(\textcolor{blue}{\textbf{-4.4}})}\\%[0.5ex]
% % Flops Saving (in \%) & 2.7 &  2.7 &  9.0 & 4.4   \\ 
% \bottomrule     
% \end{tabular}
% % \caption{Top-1 accuracy for various models trained on long tailed Imagenet and iNaturalist'18 datasets. Numbers in parenthesis indicate the flops expended by each method relative to the baseline. Whenever absent, assume 0\% flops saving. \method consistently improves accuracy while expending fewer flops. }
% % \label{tab:large_scale_results}
% % \end{table}






% \begin{table}[]
% \centering
% \begin{tabular}{lcccc}
% \toprule
% & \multicolumn{2}{c}{\textbf{Resnet-50}} & \multicolumn{2}{c}{\textbf{Densenet-169}} \\ 
% \cmidrule(l){2-3}\cmidrule(l){4-5}
% Loss type& Error & TFlops & Error & Tflops \\ 

% \midrule
% CE            & 51.5     &   205       & 52.1  &  169        \\
% EEL (CE)    & 51.0     &   163    & 51.2  &    155           \\
% \midrule
% LDAM          & 51.2   &     205       & 51.2   &  169             \\
% EEL (LDAM)  & 49.2   &     190    & 49.2   &     167          \\
% \bottomrule


% \end{tabular}
% \caption{Top-1 error and Tera Flops on the Imagenet-LT validation set. \method improves accuracy while reducing flops \rd{}}
% \label{tab:loss_type_ablation}
% \end{table}
